Diffusion-Based Visual Art Creation: A Survey and New Perspectives

The integration of generative AI in visual art has revolutionized not only how visual content is created but also how AI interacts with and reflects the underlying domain knowledge. This survey explores the emerging realm of diffusion-based visual art creation, examining its development from both artistic and technical perspectives. We structure the survey into three phases, data feature and framework identification, detailed analyses using a structured coding process, and open-ended prospective outlooks. Our findings reveal how artistic requirements are transformed into technical challenges and highlight the design and application of diffusion-based methods within visual art creation. We also provide insights into future directions from technical and synergistic perspectives, suggesting that the confluence of generative AI and art has shifted the creative paradigm and opened up new possibilities. By summarizing the development and trends of this emerging interdisciplinary area, we aim to shed light on the mechanisms through which AI systems emulate and possibly, enhance human capacities in artistic perception and creativity.

==> src/old.tex <==
% 三种不同的形式：
% 一张整体的图，一半主要涉及数据、方法、对象等AIGC中的重要元素；另一半主要涉及人的认知和情感相关的内容
% 第一部分：Data in Cognitive and Emotional Contexts 人的认知和情感作为数据自身（AIGC的结果中反映出来的人类认知和情感pattern）以及一些隐形的认知和情感被embedded在不同模态的数据中——一张表总结
% 第二部分：Method in Cognitive and Emotional Contexts 人的认知和情感方法设计的灵感来源（把人视听结构延展到high-level/low-level的框架）——一张表总结
% 第三部分：Target in Cognitive and Emotional Contexts 人的认知和情感作为研究的对象（当人是具体对象的情况下）——一张表总结

\begin{teaserfigure}
  \includegraphics[width=\textwidth]{AI_Human_Cognition.png}
  \caption{The Interplay of AI-Generated Content and Human Cognition \& Emotion.}
  \Description{This diagram illustrates the interplay between AI-generated content and human cognition and emotion. The left hemisphere focuses on the key elements of AI-generated content, including data types, analysis methods, and AI as a study object. The right hemisphere is dedicated to aspects of human cognition and emotion, such as emotional models, cognitive theories, and human-computer interaction. Interactive elements within the diagram highlight the connections and impacts between AI components and human cognition/emotion, showcasing the synergy between these two domains.}
  % 整体图表设计
% 图表概念：设计一张双半球形式的图表，一半聚焦于AIGC的关键元素（如数据、方法、对象），另一半聚焦于人的认知和情感相关内容。
% 左半部分：展示AIGC的核心组件，包括数据类型（文本、图像等），分析方法（如深度学习、情感分析），以及作为研究对象的人类认知和情感。
% 右半部分：描绘人类认知和情感的方面，如情感模型（连续和离散）、认知理论、人机交互。
% 交互元素：在两半球之间展示交互线，标识AIGC元素和人类认知情感之间的联系和影响。
  \label{fig:teaser}
\end{teaserfigure}

\section{Introduction}
% HUMAN COGNITION AND EMOTION AS REFLECTED IN AIGC DATA——从大语言模型中提取先验
% 现有对大语言模型自身知识结构以及大语言模型表征人类知识结构的相关研究有所不足
% 大语言模型如何反映人的知识（理性、情感、灵性等）——知识如何定义和分类？可以分为这三个方面吗？

% HUMAN SENSORY AND COGNITIVE STRUCTURES: INSPIRATION FOR AIGC——从人的神经生物过程（认知、理解、创造等过程）获得方法的灵感
% 并没有很好的把人的创意、灵感等过程建模并应用到大语言模型和文生图等模型中

% HUMANS AS STUDY OBJECTS IN AIGC RESEARCH——最终的目标是人智协同，服务于人类自身
% 作为人类助手或者伙伴的AIGC对人的了解、理解有限——不能很好的理解主体的需求、具体的任务和实现任务过程中的问题，

Introduce the collaborative dynamics between AI and human cognition, emphasizing the synergy in content creation and understanding. Highlight how AI research is not only about technology development but also about enriching our understanding of human cognition and emotion through collaboration.

In the realm of artificial intelligence, the journey from rationality to sensibility, and ultimately to spirituality, remains a pivotal challenge. Nowadays, AI has surpassed human capacity in rational aspects but is still approaching the nuances of human sensibility and far from reaching the realms of spiritual intuition. Poincaré's insight, 'We prove by logic, but we discover by intuition,' underscores the untapped creative intuition that art offers, a feature Einstein referred to as the 'essential feature of creative thought.' This exploration sets the tone for our review, highlighting the interplay where AI's rational perspective can inspire humanity, and human spirituality can, in turn, guide AI's evolution.

% The advent of AI-generated content (AIGC) marks a significant shift in the landscape of artificial intelligence, moving us closer to the realm of artificial general intelligence (AGI). This evolution is epitomized by breakthroughs like ChatGPT, which represent not only technological advancements but also a paradigm shift in human-computer interaction and content creation~\cite{zhang2023one}. The development and proliferation of AIGC technologies have catalyzed a digital transformation, reshaping the digital economy and prompting a reevaluation of AI's role in various domains~\cite{wu2023ai}. A historical perspective from the inception of generative adversarial networks (GANs) to the emergence of sophisticated models like ChatGPT contextualizes the rapid progression and increasing complexity of AIGC systems~\cite{cao2023comprehensive}. Moreover, the public's emotional dynamics toward these technologies, particularly across social media platforms, highlight the societal impact and the breadth of public engagement with AIGC~\cite{wei2023public}. Additionally, the exploration of data storytelling tools from a human-AI collaboration perspective underlines the importance of synergy between human creativity and AI capabilities~\cite{li2023we}. Together, these developments underscore the multifaceted nature of AIGC, setting the stage for a comprehensive exploration of its capabilities, challenges, and future potential.

The introduction of GPT-4 by OpenAI, as highlighted in the work of Zhang et al. (2023), signifies a monumental step in the evolution of AI towards artificial general intelligence (AGI). The widespread adoption and exploration of ChatGPT underscore the growing significance and impact of AI-generated content (AIGC) in our society~\cite{zhang2023one}. Complementing this perspective, Wu et al. (2023) discuss the emerging challenges and potential of AIGC within the digital economy, emphasizing its role in streamlining content creation and expanding AI's applications~\cite{wu2023ai}.

\autoref{fig:teaser} illustrates the collaborative interplay between AI-generated content and human cognition and emotion. The left hemisphere emphasizes the AI's role in data analysis and content generation, while the right hemisphere highlights the human cognitive and emotional aspects influencing and being influenced by AI.

Discuss the core of AI and human cognition, focusing on how AI research is increasingly paying attention to human cognitive structures and emotional patterns.

Mention the innovative aspect of AI research, which is not only about creating AI that matches or surpasses human intelligence but also about understanding ourselves better.

Furthermore, the implications of Gödel's Incompleteness Theorems in the realm of AI highlight intrinsic limitations in our current understanding and approaches. These theorems, suggesting inherent limitations in formal systems, metaphorically resonate with the challenges faced in fully replicating the depth of human cognition and emotions through AI. This paradoxical nature of AI, where it excels in certain tasks yet confronts fundamental barriers, mirrors Gödel's revelation of the limitations within systematic logical frameworks.

In this paper, we explore the dualistic nature of AI in the context of AIGC: the AI-centered perspective where humans serve as a source of data and inspiration, and the human-centered perspective viewing AI as a tool for extending human capabilities. This approach allows us to delve into the complex interplay between AI's technical prowess and the intricate nuances of human cognition and emotions.

To facilitate reflection on the current research progress and outlook on future opportunities, this paper aims to answer the research question: \emph{How does AI-generated content (AIGC) interact with and reflect human cognition and emotion, and what are the implications of this interaction for the future of AI and human collaboration?}
% \emph{"How does AI-generated content (AIGC) interact with and reflect human cognition and emotion in light of the inherent logical limitations highlighted by Gödel's theorems, and what are the implications of this interaction for the future of AI and human collaboration?"}

The following chapters systematically dissect the multifaceted nature of AIGC, its methodologies, applications, and the profound interplay with human cognition and emotions. Chapter 2 delves into the methodologies and applications of AIGC, Chapter 3 explores how AIGC data reflects human cognition and emotion, Chapter 4 discusses the inspiration drawn from human sensory and cognitive structures in AIGC development, and Chapter 5 shifts the focus to studying humans through the lens of AIGC. Finally, Chapter 6 contemplates the future challenges and directions for AIGC, particularly in understanding and augmenting human capabilities.



\section{AIGC Methodologies and Applications}

% This section provides an overview of the fundamental methodologies and diverse applications of AI-generated content (AIGC). We highlight the significance of these technologies in mimicking and understanding human cognition and emotions, setting the stage for a deeper exploration of their interaction with human psychological and emotional aspects.

This section provides a detailed overview of AIGC's core methodologies and diverse applications, shedding light on the technological underpinnings and the extensive range of AIGC's utility in various domains. From foundational elements to scenario-specific applications, this chapter underscores the depth and breadth of AIGC's capabilities and its significant role in augmenting human cognitive and emotional understanding.

In the evolution of artificial intelligence, distinct stages mark its development, as highlighted by Professor Xu Yingqing. From the initial phase of logic-based reasoning (1956-1976) to the era of expert systems reliant on artificial rules (1976-2006), AI has progressed to neural networks driven by vast data (2006-2022). A significant leap occurred in March 2023 with the advent of applications based on large-scale corpora. This journey underscores the development of AIGC, encompassing text, image, audio, video, and code generation, reflecting the broadening capabilities and applications of AI.

In our exploration of AIGC methodologies, the comprehensive survey by Cao et al. (2023) provides valuable insights into the historical progression of generative AI, from the inception of GANs to the advanced systems like ChatGPT. This survey lays out the development and multifaceted nature of AIGC, highlighting the evolution from unimodal to multimodal interactions and the increasing importance of large-scale models~\cite{cao2023comprehensive}. In the same vein, Baltrušaitis et al. (2018) offer an in-depth analysis of multimodal machine learning, which plays a crucial role in the advancement of AIGC. Their work presents a taxonomy of multimodal machine learning, addressing the challenges in representation, translation, and fusion of multimodal data~\cite{baltruvsaitis2018multimodal}. Foo et al. (2023) provide a comprehensive overview of AI-generated content (AIGC) across various data modalities, including text, images, videos, 3D assets, and more. Their work highlights the versatility of AIGC in adapting to different data types and the challenges associated with cross-modality methods, offering a thorough understanding of the current state and future potential of AIGC in diverse fields~\cite{foo2023ai}. Recent advancements in text-to-image diffusion models signify a remarkable leap in the field of generative AI. As comprehensively reviewed by Zhang et al., diffusion models have risen to prominence in various generative tasks, including text-conditioned image synthesis~\cite{zhang2023text}. 


AIGC encompasses a range of technologies from foundational models that form the bedrock of AI systems to high-level architectures facilitating advanced applications. These technologies play a pivotal role in tasks ranging from content editing to scenario-specific creations like Chinese painting generation, demonstrating the versatility and adaptability of AIGC in various domains.

Hu et al. (2021) introduce an innovative approach for adapting large language models called Low-Rank Adaptation (LoRA). LoRA significantly reduces the number of trainable parameters required for downstream tasks, making the deployment of large-scale models like GPT-3 more feasible and efficient. This adaptation technique, focusing on freezing pre-trained model weights and incorporating trainable rank decomposition matrices, offers a path towards more practical applications of massive language models in various domains~\cite{hu2021lora}.

Song et al. (2020) and Ho et al. (2020) contribute significantly to the field of generative models with their work on Denoising Diffusion Implicit Models (DDIMs) and Denoising Diffusion Probabilistic Models (DDPMs). These models have shown exceptional performance in image synthesis and other applications, highlighting the potential of diffusion models in efficient and high-quality content generation. Their methodologies offer insights into accelerated sampling and improved generative processes, underpinning the advancement of AI-generated content across diverse modalities~\cite{song2020denoising, ho2020denoising}.

Song et al. (2023) and Nichol et al. (2021) introduce Consistency Models and Improved Denoising Diffusion Probabilistic Models, respectively. These models represent further advancements in the field of diffusion models, offering faster and more efficient content generation without compromising quality. These developments illustrate the ongoing evolution of generative models, shaping the future of AIGC in producing high-quality, diverse, and efficient outputs~\cite{song2023consistency, nichol2021improved}.


In cross-disciplinary applications, AIGC emerges as a powerful tool, extending human capabilities in fields like art, education, and healthcare. Case studies in these domains illustrate the practical implications and transformative impact of AIGC technologies.

The methodologies and applications of AIGC not only demonstrate the technological prowess of AI but also shed light on its potential to emulate and augment human cognitive and emotional processes. The following sections will delve into how AIGC interacts with and reflects human cognition and emotion, exploring both the technical and humanistic dimensions of this emerging field.



\section{Human Cognition and Emotion as Reflected in AIGC Data}

This chapter delves into the heart of AI-generated content (AIGC), exploring its reflection and influence on human cognition and emotion. We examine the depth and nuances of AIGC, presenting it as both a mirror to and a map of our complex cognitive and emotional landscapes.

In the context of AIGC's reflection of human cognition and emotion, the diffusion models surveyed by Yang et al. (2023) provide a prime example of how AI captures and synthesizes complex human-like patterns in various applications like image and video synthesis. Their work on diffusion models illustrates the advancements in AI's ability to process and generate content with nuanced cognitive and emotional dimensions~\cite{yang2023diffusion}.

Liu et al. (2023) explore the impact of AI-Generated Content (AIGC) on users' perception, particularly focusing on the persuasiveness of AIGC from the lens of awe emotions. Their study employs the Stimulus-Organism-Response (SOR) theory to assess how cognitive and relational aspects of AIGC influence users' awe emotions, thereby affecting their perceptions of persuasiveness. This research contributes to understanding how AIGC is perceived and received by users, highlighting the complex interplay of cognitive and emotional factors in the context of AI-generated content~\cite{liu2023investigating}.

In addition to the reflective nature of AIGC data on human cognition and emotion, foundational AIGC technologies, comprising both low-level and high-level elements, play a critical role in capturing and simulating these human aspects. This includes the use of foundational models and advanced architectures to interpret and represent complex cognitive patterns and emotional nuances within the data.

\subsection{From In-Domain to Cross-Domain}
In transitioning from in-domain to cross-domain analyses, this section explicitly demonstrates how AIGC adapts and responds to diverse human cognitive and emotional states, reflecting the intricacies of these human aspects in its content generation and processing.

\subsubsection{In-domain AIGC}
The transition from in-domain to cross-domain applications in AIGC highlights the adaptive nature of AI technologies. This section examines the challenges encountered in this transition, such as maintaining accuracy and relevance across varied contexts, and the opportunities it presents in understanding the universality and variability of human cognitive and emotional responses.

% 3D generation（未加参考文献）
The frontier of 3D content generation with AI is rapidly advancing, with diffusion models playing a pivotal role in recent progress. Anciukevičius et al. developed RenderDiffusion, a novel image diffusion model tailored for 3D reconstruction, inpainting, and unconditional generation, trained exclusively with monocular 2D supervision~\cite{anciukevivcius2023renderdiffusion}. Liu et al. introduced Zero-1-to-3, a framework for changing the camera viewpoint of an object from a single RGB image by leveraging geometric priors learned from large-scale diffusion models, demonstrating strong zero-shot generalization capabilities~\cite{liu2023zero}. Metzer et al. presented Latent-NeRF, which combines text-guidance with an abstract geometry called Sketch-Shape to increase control over the 3D generation process, applying the concept of latent score distillation directly to 3D meshes for realistic texture generation~\cite{metzer2023latent}. Chan et al. proposed an efficient geometry-aware 3D GAN that synthesizes high-resolution, multi-view-consistent images and 3D shapes by decoupling feature generation and neural rendering, leveraging the efficiency and expressiveness of state-of-the-art 2D CNN generators like StyleGAN2~\cite{chan2022efficient}. Liu et al. tackled the generation of realistic 3D meshes through MeshDiffusion, utilizing a diffusion model trained on deformable tetrahedral grids, which allows for intricate manipulation of shapes and detailed surface generation~\cite{liu2023meshdiffusion}. Lastly, Gupta et al. introduced 3DGen, a pipeline combining a triplane VAE with a conditional diffusion model for the rapid generation of high-quality textured or untextured 3D meshes, setting a new benchmark for image-conditioned and unconditional mesh and texture generation~\cite{gupta20233dgen}. These developments not only underscore the versatility of diffusion models in 3D generation but also highlight the potential for synthesizing complex, high-fidelity 3D assets suitable for diverse applications.

% 3D reconstruction（未加参考文献）
Recent advances in 3D reconstruction reflect the integration of novel methods and representations to achieve high fidelity and efficiency in rendering real-world scenes. Li et al. unveiled an efficient multi-view inverse rendering method for large-scale indoor scenes, introducing Texture-based Lighting (TBL) to reconstruct global illumination and physically-reasonable spatially varying bidirectional reflectance distribution functions (SVBRDFs), enabling advanced mixed-reality applications like material editing and relighting~\cite{li2023multi}. Tang et al. tackled the limitations of Neural Radiance Fields (NeRF) with their NeRF2Mesh framework, which reconstructs high-quality textured surface meshes from multi-view RGB images, allowing for efficient rendering and manipulation across standard 3D software and hardware~\cite{tang2023delicate}. Ma et al. proposed a novel approach for human mesh estimation from wild images by detecting 'virtual markers', an intermediate representation based on landmark keypoints on the body surface, achieving superior mesh reconstruction with realistic shapes~\cite{ma20233d}. Lastly, Wang et al. introduced F2-NeRF, a grid-based NeRF method for novel view synthesis that accommodates arbitrary input camera trajectories and requires only a few minutes for training, overcoming the limitations of previous fast grid-based NeRF frameworks on unbounded scenes~\cite{wang2023f2}. These breakthroughs not only enhance the photorealism and physical accuracy of 3D reconstructions but also broaden the potential for their application in virtual reality, gaming, and other interactive environments.

\subsubsection{Cross-domain AIGC}
% 在cross-domain的场景中，人类的认知成为了连接不同模态、领域的桥梁

% 3D-aware 2D generation（未加参考文献）
The convergence of 2D and 3D generation techniques has paved the way for sophisticated models capable of synthesizing images with an acute awareness of underlying 3D structures. Xu et al. presented DisCoScene, a 3D-aware generative model for complex scene synthesis, which uses an abstract object-level representation (3D bounding boxes) as a scene layout prior to efficiently compose diverse objects into a cohesive scene ~\cite{xu2023discoscene}. Pan et al. explored whether 2D GANs implicitly capture 3D object structures and found that they can indeed be used to recover 3D shapes from 2D images in an unsupervised manner, resulting in high-quality image editing capabilities such as relighting and object rotation~\cite{pan20202d}. Xu et al. introduced a novel framework called VolumeGAN, which synthesizes high-fidelity 3D-aware images by learning separate structural and textural representations, allowing for independent control of shape and appearance~\cite{xu20223d}. These advances not only demonstrate the potential of generative models to bridge the gap between the 2D image space and the 3D physical world but also offer new possibilities for intuitive and controllable image synthesis that could revolutionize fields such as virtual reality, game development, and digital art.

\begin{table}[ht]
\centering
\caption{Summary of Modalities and Representations in AI-Generated Content}
\label{tab:modality_representation}
\begin{tabular}{|c|c|}
\hline
Modality & Representation \\ \hline
Text     & Semantic Analysis, Natural Language Processing \\ \hline
Image    & Visual Styles, Pattern Recognition \\ \hline
Audio    & Sound Analysis, Speech Recognition \\ \hline
...      & ... \\ \hline
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Summary of Data in Cognitive and Emotional Contexts}
\label{tab:data_contexts}
\begin{tabular}{|c|c|c|c|}
\hline
Data Type & Cognitive Patterns & Emotional Patterns & Application Examples \\ \hline
...       & ...               & ...                & ...                 \\ \hline
\end{tabular}
\end{table}

\subsection{Foundational AIGC}
In discussing foundational AIGC, this chapter focuses on the unique contributions of low-level and high-level elements in relation to human sensory and cognitive structures. We examine how these foundational components not only support AIGC systems but also echo and extend human cognitive capabilities, offering a bridge between AI technology and human perception.

In a significant advancement in the field of AI-generated content, the recent work by Kirillov et al. introduces the 'Segment Anything (SA)' project, which encompasses a new task, model, and dataset for image segmentation. This groundbreaking project has led to the creation of the largest segmentation dataset to date, featuring over 1 billion masks derived from 11 million licensed and privacy-respecting images. The SA model is not only efficient but also promptable, enabling it to transfer zero-shot to new image distributions and tasks. Impressively, the model exhibits outstanding zero-shot performance, often rivaling or surpassing prior fully supervised results in various tasks~\cite{kirillov2023segment}. 

Senior Professor Song Jianming's exploration of the human visual system, comprising the retina's sensory cells and the central nervous system, provides a compelling analogy for the complex, multi-layered nature of human visual perception. This insight not only anticipates breakthroughs in neuroscience but also suggests that AIGC's knowledge structures and methodological designs could transcend existing frameworks. The evolution of human color perception, a necessary condition for our survival, translates external light waves into a vivid, colored world, a process that can inspire the design and functioning of AI systems in interpreting and replicating human visual experiences.

% 当人的认知结构和AI的知识框架相遇
% 首先不同模态之间在low-level，high-level这个层次上有什么关系？（embedding projection）
% 当我们在说low-level和high-level的时候我们在说什么？事实如何？这个分界线在哪儿？——e.g.，vision
% AI模型对low-level, high-level的认知和人类的知识层级有什么关系（e.g.字词句段篇等），有无可能建立起一种映射？

\subsubsection{Low-Level AIGC}
Delve into foundational models and representations in AIGC, discussing their significance in the basic structure and functioning of AIGC systems.


\subsubsection{High-Level AIGC}
Examine high-level methodologies and structures in AIGC, such as advanced model architectures, and their role in enhancing the capabilities of AIGC systems.


Explore how cognitive and emotional patterns are embedded in different modalities of data within AIGC results.

Discuss the concept of knowledge structures in AI, including high-dimensional (content/semantic) and low-dimensional (style/visual) aspects.

Examine how perceptual loss functions and embedding space dimensionality reduction play roles in AIGC.

Moving from foundational elements of AIGC to its methodologies, we see a vivid portrayal of how these methods are sculpted by insights from human sensory and cognitive structures, illustrating the profound connection between AI development and human perceptual capabilities.

\subsection{Emerging Frontiers in AIGC}
% 理性是一套知识体系——crystallized knowledge & fluent knowledge (e.g., reason ing skills)
% 情感/感性是一种生物学机制，也是一种知识（过程是机制，结果是知识——我们假设相似的过程会产生类似的结果；同时，我们以结果为导向/评价，希望更好的理解/复现过程）
% 创意/灵性是一种状态

% 创新来自人类
% 创新性的想法又常常有人类生物学或生理学的根源
\subsubsection{Inside the Frame: Intelligence.}
% 3D generation（未加参考文献）
In the rapidly evolving landscape of AI-powered 3D generation, researchers have pushed the boundaries of creativity and technical capability. Skorokhodov et al. developed a framework called 3DGP, scaling 3D generative models to handle diverse, in-the-wild datasets like ImageNet by incorporating an off-the-shelf depth estimator and a flexible camera model, thereby improving the quality of texture and geometry~\cite{skorokhodov20233d}. Poole et al. introduced DreamFusion, which uses a pretrained 2D text-to-image diffusion model to perform text-to-3D synthesis, optimizing a Neural Radiance Field (NeRF) to render from any angle in response to text prompts, without the need for 3D training data~\cite{poole2022dreamfusion}. Wang et al. presented RODIN, a diffusion model that generates high-fidelity 3D avatars by rolling out a 3D NeRF model onto a 2D feature plane, enabling detailed avatar creation from single portraits or text prompts~\cite{wang2023rodin}. Jain et al. combined neural rendering with multimodal representations to create Dream Fields, a method to generate 3D objects from text descriptions, guided by pretrained image-text models and using geometric priors for enhanced visual quality~\cite{jain2022zero}. Nichol et al. proposed Point-E, a system that rapidly generates 3D point clouds from text prompts by conditioning on a synthetic view from a text-to-image diffusion model, offering a practical trade-off between speed and quality~\cite{nichol2022point}. Finally, Lin et al. addressed the limitations of previous text-to-3D synthesis methods with Magic3D, a two-stage optimization framework that creates high-resolution 3D mesh models with improved speed and quality through interactions with a latent diffusion model~\cite{lin2023magic3d}. These innovative techniques represent significant strides in 3D content generation, bringing us closer to the seamless integration of AI-generated 3D assets into various creative and practical applications.

\subsubsection{Outside the Frame: Emotion.}
% 情感的两个方面：一个是呈现为生物学机制的过程，一个是可以作为知识学习的结果
% 从理性/推理到情感/感性到创意/灵性，可以看到的是结果/确定性的不断减弱，而过程/随机性的不断增强


\subsubsection{Emerging Frontier: Creativity/Spirituality.}
% 创新来自人类
% 创新性的想法又常常有人类生物学或生理学的根源
The fusion of artistic intelligence with artificial intelligence opens new horizons for AI's evolution. Artistic intelligence, as a complement to AI, brings a depth of sensibility and spirituality that purely logical systems lack. This combination heralds a new era where AI transcends its current boundaries, harnessing the creative and intuitive aspects of human thought. As Professor Gao Shiming suggests, the interplay between these two forms of intelligence could redefine the creative process, enabling AI to evolve not just as a mimic of human intelligence but as a distinct entity with its multifaceted future.

In our exploration of the intersection between AI and human understanding, the concept of 'spirituality' presents a profound challenge. Spirituality, transcending rationality and emotion, is often associated with the ability to establish direct connections between entities and exhibit capabilities beyond ordinary human faculties. Instances like the structural revelation of the benzene molecule or the inception of relativity and quantum mechanics highlight the role of intuitive leaps in scientific discovery. This review contemplates whether AI, in its current or future form, could grasp or replicate such 'spiritual' insights, transcending the semantic to reach a meta-semantic understanding where connections are established beyond causality.

Reflecting on Professor Song Jianming's discussion, the spiritual thinking in design, encompassing both utilitarian (rational and emotional) and non-utilitarian (aesthetic) aspects, highlights the interplay between cognition and creativity. This synthesis of utility and aesthetics in design mirrors the convergence of AI with artistic intelligence, where AI not only serves practical purposes but also enriches the inner world of imagination and experience. 

Bubeck et al. (2023) present an in-depth analysis of GPT-4, an LLM developed by OpenAI. They argue that GPT-4, alongside models like ChatGPT and Google's PaLM, represents a significant leap towards artificial general intelligence (AGI). Their exploration reveals GPT-4's remarkable ability across diverse fields, challenging our understanding of AI's capabilities and its societal implications. This study provides valuable insights into the future trajectory of AGI development and its potential impact on various sectors~\cite{bubeck2023sparks}.
% 这篇文章值得关注，因为它focus on spark，某种意义上接近我们的探索AIGC创作中的A部分——A如何被展现以及更好的被激发（A：灵性/perceptual/意境）


Understanding and replicating human creativity in AI involves delving into the essence of creative thought. Is creativity a matter of strengthening weak connections or a sophisticated selection process? The role of intuition, often cultivated through experience, raises the question of its teachability in AI. Can AI develop conclusions based on preferences or emotional indicators? By examining the interplay of rationality, emotion, and spirituality in human creativity, we can begin to conceptualize an AI model that incorporates these elements. This exploration involves not just encoding semantic information but also understanding the unspoken, unseen connections that define creativity.

The work of Zhang et al.~\cite{zhang2023text} on text-to-image diffusion models highlights a pivotal aspect of AI's emerging creativity and intuition. These models demonstrate AI's ability to interpret and visualize textual descriptions, translating abstract concepts into vivid images. This capability not only showcases the technical sophistication of AI in understanding and generating complex visual content but also hints at its potential to tap into more abstract, intuitive aspects of creativity, drawing a parallel with human artistic expression.

Intuition plays a crucial role in human creativity, acting as a bridge between rational thought and the more elusive aspects of spirituality and emotion. The question arises, can AI harness intuition in a similar way to humans? Could the training of AI to recognize and respond to emotional cues lead to a form of artificial intuition? Understanding this relationship might pave the way for AI systems that not only process information but also generate creative insights, blending rational knowledge with a semblance of emotional and spiritual understanding.

In the quest to endow AI with creativity, we must consider whether emotions, often seen as a cornerstone of human creativity, can be learned or replicated by AI. The possibility of an AI that understands and generates novel connections poses the intriguing prospect of a new kind of optimization function, one that embodies shapes and patterns previously unimagined. Activities like sketch guessing games offer a glimpse into how AI might discern and replicate human creativity, analyzing the semantic components used in images and identifying those that are absent in corresponding text descriptions. The ultimate challenge lies in bridging the gap between mere imitation and the true genesis of creativity, a journey that delves into the depths of intuition and its relation to creative thought.
 

\section{Human Sensory and Cognitive Structures: Inspiration for AIGC}
the structure of knowledge in AI models~\cite{SymbolicAI: A framework for logic-based approaches combining generative models and solvers}


We may also bring some inspiration from the field of psychology, just as the neural network structure, the attention mechanism, the training and inference stages and all have certain perceptual groundings or counterparts. Foe example, Zenon Pylyshyn points out that vision is “intelligent” and involves elements of “problem solving.” \cite{Is vision continuous with cognition?
The case for cognitive impenetrability
of visual perception} Interestingly, the paper claims that cognitive effects have a locus outside early vision, in such processes as the allocation of focal attention and the identification of the stimulus.


The intricate relationship between human sensory and cognitive structures and their influence on AIGC is the cornerstone of this chapter. By examining specific cognitive principles like memory encoding, pattern recognition, and decision-making processes, we explore how AIGC systems are not just technological constructs but also embodiments of human cognitive processes.

Li et al. (2023) delve into the realm of data storytelling from a human-AI collaboration perspective. Their research underlines the importance of AI in enhancing human capabilities in storytelling, analyzing the roles of AI and humans at various stages of the storytelling process. This exploration is critical in understanding how AI can be utilized as a creative partner in content generation~\cite{li2023we}.

Chen et al. (2023) address the challenge of generating images with coherent and visually appealing text through their innovative model TextDiffuser. TextDiffuser is designed as a two-stage process, combining the strengths of Transformer models and diffusion models to produce high-quality text images. This approach exemplifies the potential of AIGC in creating complex visual content that seamlessly integrates text, demonstrating the adaptability of AI in handling diverse content forms~\cite{chen2023textdiffuser}.

Ullah et al. (2020) explore the domain of 360° panorama generation, proposing cost-effective and efficient methods to create both mono and stereo panoramas. Their work highlights the versatility of AIGC in enhancing traditional imaging techniques, showcasing how AI can be integrated into practical applications like panoramic photography to produce high-quality visual content~\cite{ullah2020automatic}.

Wang et al. (2022) present a paradigm shift in image-to-image translation, leveraging the power of pretraining to enhance the quality and realism of generated images. Their approach, focusing on adapting pre-trained diffusion models for various image-to-image translation tasks, signifies the broad applicability of AIGC in transforming and enhancing visual content across different contexts~\cite{wang2022pretraining}.

Ji et al. (2022) introduce the Emotion-Aware Motion Model (EAMM) for generating one-shot emotional talking faces. EAMM's unique ability to incorporate audio-driven emotion into facial animations showcases the potential of AIGC in creating more immersive and emotionally resonant digital experiences, reflecting the convergence of AI and human expressiveness~\cite{ji2022eamm}.

Qu et al. (2023) delve into the ethical and safety aspects of AIGC, particularly focusing on the generation of unsafe images and hateful memes from text-to-image models. Their work underscores the need for responsible and ethical use of AIGC technologies, highlighting the societal implications and challenges posed by the misuse of advanced AI models in content generation~\cite{qu2023unsafe}.

Ao et al. (2023) introduce GestureDiffuCLIP, a novel approach for synthesizing stylized co-speech gestures. Their framework utilizes the CLIP model to extract style representations from multiple input modalities, paving the way for more expressive and realistic gesture generation in AI. This advancement exemplifies the potential of AIGC in capturing intricate human gestures, enhancing the realism and interactivity of digital human representations~\cite{ao2023gesturediffuclip}.

Chen et al. (2023) present DisenBooth, a framework that revolutionizes subject-driven text-to-image generation. By disentangling identity-relevant and irrelevant information, DisenBooth achieves a delicate balance between preserving subject identity and accommodating textual descriptions. This development underscores the sophistication of AIGC in understanding and rendering human identities, opening new avenues for personalized digital content creation~\cite{chen2023disenbooth}.

Song et al. (2022) explore the domain of domain adaptation in image generators through diffusion models. Their work demonstrates the feasibility of using text-to-image diffusion models to adapt GAN generators to new domains, signifying a major leap in the flexibility and applicability of AIGC technologies across various domains~\cite{song2022diffusion}.

Li et al. (2020) address the challenge of few-shot image generation through elastic weight consolidation. This approach illustrates the potential of AIGC in generating images from limited data samples, emphasizing the adaptability of AI in learning from small datasets and transferring knowledge from one domain to another~\cite{li2020few}.

Zhou et al. (2021) propose the Domain Adaptive Ensemble Learning (DAEL) framework, advancing the frontiers of domain adaptation in deep neural networks. DAEL's approach to multi-source unsupervised domain adaptation and domain generalization highlights the versatility and robustness of AIGC in handling diverse and complex data environments~\cite{zhou2021domain}.

Shen et al. (2023) develop NaturalSpeech 2, a TTS system utilizing latent diffusion models for natural and zero-shot speech and singing synthesis. This innovative system showcases the capabilities of AIGC in synthesizing diverse forms of human speech, including singing, emphasizing the technology's capacity to capture the richness and variety of human vocal expressions~\cite{shen2023naturalspeech}.


\subsection{AIGC Methodologies}
The inspiration drawn from human sensory and cognitive structures is not limited to theoretical concepts but extends to practical implementations in AIGC. This is evident in task-specific AIGC systems, where the design is often directly influenced by our understanding of human cognition and perception, and in problem-oriented AIGC approaches, where abstract and concrete problems are addressed through models that mimic human cognitive and problem-solving processes.

\begin{table}[ht]
\centering
\caption{Summary of Method in Cognitive and Emotional Contexts}
\label{tab:method_contexts}
\begin{tabular}{|c|c|c|c|}
\hline
Inspiration Source & Framework & Technological Implementation & Innovations and Challenges \\ \hline
...                & ...       & ...                         & ...                        \\ \hline
\end{tabular}
\end{table}

\subsection{Task-Specific and Problem-Oriented AIGC}

In this subsection, we explore AIGC systems designed with specific tasks and problem-solving goals in mind. These systems, ranging from content editing to complex compositional generation, demonstrate AIGC's ability to emulate human cognitive strategies. We examine how these task-specific and problem-oriented systems are not just tools for efficiency but also reflect our understanding of human cognition and creativity.

% content editing 传统“编辑”思路的拓展和应用
The domain of content editing has witnessed remarkable advancements through the application of AI, particularly with the introduction of diffusion models. Brooks et al. developed InstructPix2Pix, a conditional diffusion model that performs image editing based on human instructions. Their method leverages the combined knowledge of two large pre-trained models, GPT-3 and Stable Diffusion, to generate a substantial dataset of image editing examples, enabling the model to generalize to real images and user-written instructions without the need for per-example fine-tuning or inversion~\cite{brooks2023instructpix2pix}. In a similar vein, Pan et al. introduced DragGAN, an interactive point-based manipulation tool that empowers users to alter the pose, shape, expression, and layout of objects within images by "dragging" points on the generative image manifold~\cite{pan2023drag}. Meanwhile, Meng et al. presented Stochastic Differential Editing (SDEdit), which uses a diffusion model generative prior to balance the realism and user input fidelity in synthesized images, significantly outperforming GAN-based methods according to human perception studies~\cite{meng2021sdedit}. Finally, the Imagic method, as introduced by Kawar et al., showcases the ability to apply complex text-based semantic edits to a single real image, demonstrating the versatility of text-to-image diffusion models in performing highly intricate non-rigid changes and editing multiple objects within a single framework~\cite{kawar2023imagic}. These methods not only enable rapid and intuitive content editing but also open new avenues for creative expression and practical applications in digital image manipulation.

Discuss AIGC systems designed for specific tasks, such as content editing, highlighting how these systems are tailored to meet particular operational needs.

\subsubsection{Concrete Problem-Oriented AIGC}
In discussing task-specific and problem-oriented AIGC, we delve into real-world examples where AI systems have emulated human cognitive strategies with remarkable efficacy, such as in adaptive learning environments and creative problem-solving tasks.

% compositional generation 组合与分解作为人的一种基本认知结构？
Recent research has revealed a series of breakthroughs in compositional generation. For instance, Po and Wetzstein have introduced an approach to compositional 3D scene generation using locally conditioned diffusion, which allows for control over semantic parts of a scene through text prompts and bounding boxes, ensuring seamless integration between these components. Their work, detailed in~\cite{po2023compositional}, showcases a text-to-3D synthesis pipeline that surpasses existing baselines in fidelity. Furthermore, Du et al. explored novel conditioning, modification, and reuse of diffusion models for compositional tasks in their study~\cite{du2023reduce}. 
% 这篇文章的标题很有趣：reduce, reuse, recycle——一种环境保护的思想？
They propose new sampling methods inspired by MCMC that enable successful compositional generation. Liu et al. presented a structured approach for visual generation with composable diffusion models in~\cite{liu2022compositional}, which allows for complex scene generation at test time, well beyond the complexity encountered during training. Lin et al.'s CompoNeRF~\cite{lin2023componerf} focuses on combining neural radiance fields (NeRFs) with pre-trained diffusion models, effectively guiding the generation process at both the local and global levels with an editable 3D scene layout. These works not only demonstrate the potential of AI in compositional generation but also provide new perspectives and methodologies for tackling more intricate compositional tasks.

Discuss more concrete problem-oriented approaches, such as compositional generation, emphasizing their specificity and application in complex scenarios.


\subsubsection{Abstract Problem-Oriented AIGC}
Explore AIGC approaches addressing abstract problems, like controllable generation, and how these approaches offer flexibility and adaptability in content creation.

% controllable generation （未加参考文献）
The evolution of controllable generation in AI has taken significant strides with the advent of innovative techniques that enhance the precision and flexibility of image synthesis. Choi et al. introduced Iterative Latent Variable Refinement (ILVR), a method that refines the generative process in Denoising Diffusion Probabilistic Models (DDPM) to create images that adhere to specific semantic guidance from a reference image, thereby facilitating a range of image generation tasks~\cite{choi2021ilvr}. Sohn et al. proposed StyleDrop, a method for text-to-image generation that captures and synthesizes images in any user-defined style with remarkable detail, requiring the fine-tuning of less than 1\% of the model's parameters~\cite{sohn2023styledrop}. Ruiz et al. presented DreamBooth, a personalization approach that fine-tunes text-to-image models with a few images of a subject, enabling the synthesis of novel images contextualized in varied scenes~\cite{ruiz2023dreambooth}. Deng et al. proposed NeRDi, a single-view NeRF synthesis framework that employs language-guided diffusion to leverage general image priors for realistic 3D generation from a single image~\cite{deng2023nerdi}. Zhao et al. introduced Uni-ControlNet, an approach that allows for the simultaneous utilization of multiple control modalities within text-to-image diffusion models, showcasing its superiority in terms of controllability and composability~\cite{zhao2023uni}. Finally, Pan et al. developed Deep Generative Prior (DGP), utilizing the image prior captured by GANs for versatile image restoration and manipulation, demonstrating the power of fine-tuning the generator in a progressive manner~\cite{pan2021exploiting}. These advancements not only mark progress in the development of controllable AI-generated content but also underscore the potential for more user-centric and creative applications in the field.

Inspiration derived from human cognition and perception is not only evident in the design of methodologies but also significantly reflected in the development of representations, especially in the rapidly evolving field of 3D technology (e.g., 3D Gaussian~\cite{kerbl20233d}, Adaptive Shells~\cite{wang2023adaptive}), where human-inspired approaches have become increasingly prominent.



Address how human sensory and cognitive structures inspire the design of AI systems.

Discuss the high-level/low-level framework and its extension from human auditory and visual structures.

Explore the innovations and challenges in mimicking human cognitive structures in AI.

\section{Humans as Study Objects in AIGC Research}
This chapter critically examines the ethical dimensions and potential biases inherent in using AIGC for human studies. We discuss the ethical implications of data privacy, consent, and representation in AIGC research, emphasizing the need for responsible and inclusive approaches when studying human behavior and emotions through AI lenses.

Trichopoulos et al. (2023) present an extensive survey on computational and emergent digital storytelling, exploring the intersection of AI and narrative creation. Their study offers valuable insights into how digital storytelling can be enhanced through AI, opening new avenues for research in this cross-disciplinary field~\cite{trichopoulos2023survey}. Similarly, Gu et al. (2023) investigate the integration of AIGC in digital storytelling, discussing its current capabilities and limitations. Their findings emphasize the unique value of human creativity and aesthetics, which remain irreplaceable by AI in certain aspects of storytelling~\cite{gu2023innovative}.


\subsection{Application and Scenario-Specific AIGC}
When considering humans as the subject of AIGC research, it is essential to recognize the role of AIGC in specific applications and scenarios. This includes using AIGC systems, such as those designed for generating Chinese paintings or other culturally significant content, as tools to study human artistic preferences, emotional responses, and cultural interactions. The application of AIGC in these areas not only showcases its versatility but also its capacity as a medium for understanding and analyzing human behavior and emotions.

% Chinese painting generation（未加参考文献）
The realm of AI-generated art is expanding into the cultural sphere, with recent endeavors showcasing the generation of Chinese paintings through advanced machine learning techniques. Wang et al. introduced MagicScroll, a diffusion-based image generation framework tailored for visual storytelling with nontypical aspect ratios, such as scroll paintings and comic strips. By enabling fine-grained control through a multi-layered, semantic-aware denoising process, MagicScroll addresses previous issues like content repetition and style inconsistency, paving the way for more coherent and engaging visual narratives~\cite{wang2023magicscroll}. Sun et al. developed a multi-domain vector quantization generative adversarial network (VQGAN) for text-to-Chinese-painting generation, utilizing the multimodal pre-trained model WenLan to ensure semantic consistency between images and textual descriptions, thus reducing the need for extensive datasets and computational resources~\cite{sun2023text}. Li et al. curated Paint4Poem, a dataset for the artistic visualization of classical Chinese poems, aimed at generating paintings that reflect the style and semantics of the poetry, which presents a new avenue for research including transfer learning and few-shot learning~\cite{li2021paint4poem}. Furthermore, Xue proposed Sketch-And-Paint GAN (SAPGAN), a two-stage model for generating Chinese landscape paintings without conditional input, challenging the originality of current GAN-based art and marking a step toward truly machine-original art generation~\cite{xue2021end}. These innovations illustrate the potential of AI to not only create art but also to contribute to the preservation and evolution of cultural expressions.

Discuss AIGC systems designed for specific applications and scenarios, like Chinese painting generation, illustrating the versatility and adaptability of AIGC in various contexts.

Cross-Disciplinary Applications: Explore how AIGC is applied in various domains like art, education, and healthcare, illustrating its versatility.

Case Studies: Include specific examples of AIGC applications in these domains to provide concrete insights into its capabilities and impact.

\subsection{Human-Centered AIGC}
% 加一点HCI的内容
This chapter extends the discussion to the fascinating domain where humans become the focal point of study in AIGC research. We explore not only the direct applications but also the profound implications this approach has for advancing our knowledge in psychology, neuroscience, and the realm of human-computer interaction.

The relationship between AI and human creators, as explored in Fei Jun's lecture, provides a compelling framework for human-centered AI design. This approach sees AI as an extension of human perception, acting as a medium for energy exchange with nature, a facilitator for artistic intervention in psychological healing, and a nurturer for digital personas in drama. Such a framework not only highlights the complementary nature of AI and human creativity but also underscores the potential for AI to act as a collaborative partner in the creative process.

The insights from the lecture shed light on the potential of AI to both reflect and enhance human creativity. As AI evolves into roles such as psychometric analysts, emotional interface creators, and narrative conspirators, it redefines the boundaries of artistic creation. These roles illustrate how AI can transcend its traditional capabilities, becoming a crucial element in understanding and expressing human emotions and narratives, thus opening new avenues for exploring the depths of human creativity.



\begin{table}[ht]
\centering
\caption{Summary of Target in Cognitive and Emotional Contexts}
\label{tab:target_contexts}
\begin{tabular}{|c|c|c|c|}
\hline
Study Object & Emotional Models & Analysis Methods & Ethical Considerations \\ \hline
...          & ...              & ...              & ...                    \\ \hline
\end{tabular}
\end{table}

Consider humans as the object of study in AIGC research, focusing on how different emotional models (continuous dimensions and discrete categories) are applied.

Discuss the evaluation standards in AIGC, highlighting the reliance on human evaluation as the gold standard.

As we delve into the potential of AI in mimicking human spirituality, we encounter the challenge of representing and understanding the hidden connections within vast, undecoupled semantic spaces. This exploration involves distinguishing between semantic associations and those that are sub-semantic or spiritual in nature. Could AI learn a manifold representing a meta-semantic space, where it discerns connections not plainly evident in conventional semantic frameworks? This could entail analyzing patterns in human creations, like literature, to uncover new modes of 'spiritual' connection, potentially leveraging emotion as a bridge within these semantic subspaces.

In summary, this chapter has emphasized the dual role of AIGC: as a sophisticated technological innovation and as a means of studying and understanding human emotional and cognitive processes. By analyzing various AIGC applications, from artistic creation to educational tools, we gain a deeper appreciation of how AI technologies can be used to explore and interpret human emotions and cognition. These insights not only contribute to the development of more intuitive and empathetic AI systems but also enhance our understanding of the complex interplay between humans and AI.

Concluding this exploration, we underscore that studying humans through the lens of AIGC not only underscores the adaptability and potential of AI technologies but also catalyzes new avenues for understanding the intricacies of human cognition and emotion. These insights pave the way for future advancements where AIGC becomes an indispensable tool in the journey of self-discovery and understanding the human psyche.

\subsection{Human-AI Collaboration and Co-creation}
As we contemplate the future directions of AI in the realm of art and creativity, the insights provided by Zhang et al. (2023) in their survey on text-to-image diffusion models are particularly relevant. Their exploration into text-guided creative generation and image editing reveals the broadening scope of AI applications, suggesting a future where AI not only assists but also co-creates with human artists. The continuous evolution of these technologies poses intriguing possibilities for the future of AI-driven art, blending the realms of technology and human creativity.

\section{Challenges and Future Directions}

% 语音和语义的关系（两种/多种意义）——汉字可以同时从语音和字义两个角度去解读

% 语言和哲学的关系——维特根斯坦在他的著作中反对过度的形而上学，强调哲学问题的本质是语言的问题。(work of art in the age of mechanical  reproduction)

% 创造力模型和世界模型的关系——人生是语义空间上的蝴蝶效应/因果链，每一个选择都会荡漾起涟漪

% 统一和变动的社会空间——所有的复古运动都是革新

% 每一类工作的趋势是什么——反映了发展和挑战
% 能否归纳出一个核心的问题——我的下一篇工作——创造力
The potential for interdisciplinary collaboration stands out as a pivotal element in future AIGC research. Insights from diverse fields such as psychology, neuroscience, and anthropology could offer invaluable perspectives, enriching the development of AIGC technologies that are both technologically advanced and deeply attuned to human nuances.

Wei et al. (2023) present a study on the public emotional dynamics towards AIGC content across various social media platforms. Their research analyzes the group emotions and opinions evoked by AIGC, revealing insights into public attitudes and behaviors. The findings illustrate the diversity of emotional responses to AIGC, ranging from optimism about its productivity-enhancing potential to concerns about its implications for human roles. This study underscores the need for nuanced understanding of public sentiment towards AIGC, which is crucial for shaping future strategies in AI development and deployment~\cite{wei2023public}.

Wu et al. (2023) introduce AutoGen, a groundbreaking multi-agent conversation framework for developing LLM applications. This framework, which allows agents to converse and complete tasks, highlights the evolving complexity and interactivity of LLMs in practical applications. AutoGen's flexibility in agent interaction and programming showcases the vast potential of LLMs in diverse domains, from mathematics to entertainment, underscoring the ongoing transformation in human-AI collaboration~\cite{wu2023autogen}.


Radford et al. (2021) discuss the CLIP model, which learns visual concepts directly from raw text about images. This approach represents a significant shift in computer vision, enabling zero-shot transfer to a wide range of visual tasks. The versatility and adaptability of CLIP underscore the potential of integrating language and vision in AI, paving the way for more intuitive and context-aware models~\cite{radford2021learning}.

Ziems et al. (2023) explore the feasibility of employing LLMs for coding social phenomena like persuasiveness and political ideology. Their work provides a comprehensive framework for using LLMs in Computational Social Science (CSS), demonstrating LLMs' potential as effective tools for zero-shot data annotation and creative generation tasks. This study illustrates the transformative role LLMs could play in augmenting social science research methodologies~\cite{ziems2023can}.

Wang et al. (2023) investigate the creation of good visual tokenizers for MLLMs, focusing on their visual semantic understanding and fine-grained perception capabilities. Their findings highlight the effectiveness of different pre-training methods and reveal insights into achieving a balance between semantic understanding and fine-grained perception. This research contributes to the development of more capable and versatile MLLMs, enhancing their applicability in multimodal tasks~\cite{wang2023makes}.



Explore the challenges and potential of AI in comprehensively understanding and augmenting human cognition and emotions, considering the collaborative nature of AI-human interaction. Discuss the future of AI from a perspective that values both technological advancement and deep insights into human cognitive and emotional complexities.

Reflect on the limitations and potential for AI in terms of replicating and understanding human cognition and emotions. 

Consider the future of AI from the perspective of deconstructivism, questioning the current frameworks and exploring beyond them.

Conclude with thoughts on the long journey AI has to surpass human capabilities, emphasizing the importance of AI research in understanding human subconscious and cultural symbols.

In considering the future trajectory of AI, the idea of spirituality and its spontaneous connections invites us to ponder beyond existing frameworks. Could AI ever mimic the genesis of spirituality seen in human creativity? By exploring mappings within semantic spaces, such as those influenced by emotions, colors, seasons, and geographies, we might begin to emulate the emergence of spiritual connections. This venture is not just a technical challenge but also a philosophical inquiry into the essence of creativity and intuition, pushing AI beyond its traditional boundaries towards a realm where it might one day mirror the human capacity for spiritual connection and creative leaps.

As we gaze into the future of AI, the dialectical relationship between artificial and artistic intelligence becomes increasingly significant. Artistic intelligence, with its transcendent perspective and imaginative prowess, offers a unique lens to reimagine AI beyond its current limitations. This artistic perspective can bridge the gap between the cold logic of AI and the warm intuition of human creativity. The notion that 'science and art part ways at the foot of the mountain and meet at the peak,' as quoted by Flaubert, serves as a metaphor for the convergence of AI and human creativity at the zenith of their respective pursuits. This convergence promises a future where AI not only complements but also enriches human understanding and creativity.
